Domain Expansion of Image Generators

Can one inject new concepts into an already trained generative model, while respecting its existing structure and knowledge? We propose a new task - domain expansion - to address this. Given a pretrained generator and novel (but related) domains, we expand the generator to jointly model all domains, old and new, harmoniously. First, we note the generator contains a meaningful, pretrained latent space. Is it possible to minimally perturb this hard-earned representation, while maximally representing the new domains? Interestingly, we find that the latent space offers unused, "dormant" directions, which do not affect the output. This provides an opportunity: By "repurposing" these directions, we can represent new domains without perturbing the original representation. In fact, we find that pretrained generators have the capacity to add several - even hundreds - of new domains! Using our expansion method, one "expanded" model can supersede numerous domain-specific models, without expanding the model size. Additionally, a single expanded generator natively supports smooth transitions between domains, as well as composition of domains. Code and project page available at https://yotamnitzan.github.io/domain-expansion/.

==> 5_ablation.tex <==
\section{Ablation and Analysis}
\label{sec:ablation}

\textbf{Some will go to supp.}





==> 9_todo.tex <==
\myparagraph{TODO:}
\begin{todolist}
    \item Add Diffusion Autoencoder experiment.
    \item Add references suggested by R2, R3.
    \item Add NADA and MyStyle FID (to table 2?).
    \item Discuss training times somewhere.
    \item camera-ready \href{https://docs.google.com/document/d/1I-FLe5Oxfyo3OsOFTGUYxe-OpVD09bcidGF4-cAd6jw/edit#}{instructions}. 
\end{todolist}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
